On the Approximation of Functions with Line Singularities by Ridgelets

In [GO15], the authors discussed the existence of numerically feasible solvers for advection equations that run in optimal computational complexity. In this paper, we complete the last remaining requirement to achieve this goal - by showing that ridgelets, on which the solver is based, approximate functions with line singularities (which may appear as solutions to the advection equation) with the best possible approximation rate. Structurally, the proof resembles [Can01], where a similar result was proved for a different ridgelet construction, which is however not well-suited for use in a PDE solver (and in particular, not suitable for the CDD-schemes [CDD01] we are interested in). Due to the differences between the two ridgelet constructions, we have to deal with quite a different set of issues, but are also able to relax the (support) conditions on the function being approximated. Finally, the proof employs a new convolution-type estimate that could be of independent interest due to its sharpness.

==> header/header_glossaries.tex <==
\usepackage{tabu}
\usepackage{catchfile}
\usepackage[nomain,nolist,style=long]{glossaries}% last two options for compatibility with classicthesis

\newglossary[symb]{symbol}{symin}{symout}{Symbols}
\newglossary[letr]{letter}{letin}{letout}{Letters}

\glsaddstoragekey%
{origin}% key/field name
{}% default value if not explicitly set
{\origin}% custom command to access the value if required

%\glssetexpandfield{origin}% for \ref's etc.

\newglossarystyle{listofsymbols}{%
% put the glossary in the itemize environment:
\renewenvironment{theglossary}%
{%
	\tabulinesep = 2.5pt% \defaultaddspace = 5pt (use e.g. \showthe)
	\begin{longtabu} to \linewidth {lXl} \toprule%
	Symbol & Meaning & Introduced in \\ \midrule%
}{%
	\bottomrule%
	\end{longtabu}%
}%
% have nothing after \begin{theglossary}:
\renewcommand*{\glossaryname}{List of Symbols}%
\renewcommand*{\glossaryheader}{}%
% have nothing between glossary groups:
\renewcommand*{\glsgroupheading}[1]{}%
\renewcommand*{\glsgroupskip}{}%
% set how each entry should appear:
\renewcommand*{\glossentry}[2]{%
	\glstarget{##1}{\glossentryname{##1}}% the entry name
	& \glossentrydesc{##1} & \origin{##1}\tabularnewline% the number list would be in square brackets "[##2]"
}%
% set how sub-entries appear:
\renewcommand*{\subglossentry}[3]{\glossentry{##2}{##3}}% flat glossary
}

% The actual replacement mechanism
%	\@glo@sort=empty? -> use \@glo@name
% in glossaries package is hidden in the bowels of
%	\gls@assign@field -> \@gls@(no)expand@fields,
% which I didn't want to touch for fear of breaking something else.
% Conversely, this means that NO SANITATION of the sort key takes place,
% and I'm too lazy to (try to) implement that because I don't need it.
\makeatletter
\patchcmd{\gls@defglossaryentry}{\letcs\@glo@sort{glo@\@glo@label @sortvalue}}%
	{%
		\edef\tempstring{{\@glo@type}}% tex.stackexchange.com/a/24924/42225
		\expandafter\ifstrequal\tempstring{letter}%
			{% true
				\ifdefequal{\@glo@sort}{\@gls@default@value}{\let\@glo@sort\@glo@label}{}
			}%
			{% false
				\expandafter\ifstrequal\tempstring{symbol}%
				{% true
					\ifdefequal{\@glo@sort}{\@gls@default@value}{\let\@glo@sort\@glo@label}{}
				}%
				{% false
					\letcs\@glo@sort{glo@\@glo@label @sortvalue}%
				}%
			}%
	}{}{}
\makeatother

\makeglossaries

\newglossaryentry{advec_op}{
	type=letter,
	name={$A$},
	description={The main differential operator corresponding to the advection equation},
	origin={Eq. \protect\eqref{eq:LinTrans}}}
\newglossaryentry{signalclass}{%
	type=letter,
	name={$\FC$},
	sort={Csignal},
	description={A signal class, usually a (relatively) compact subset of a separable Hilbert space $\CH$},
	origin={Def. \protect\ref{def:nonlin_basics}}}
\newglossaryentry{dim}{%
	type=letter,
	name={$d$},
	description={The ambient dimension}}
\newglossaryentry{sigmastar}{%
	type=letter,
	name={$\sigma^*$},
	sort={Sz},% after other S-related stuff
	description={The optimal encoding rate for the signal class \gls{signalclass}},
	origin={Def. \protect\ref{def:encoding_rate}}}
\newglossaryentry{Rs}{%
	type=letter,
	name={$\Rs$},
	description={Rotation taking $\vec s$ into $\vec e_1$},
	origin={Def. \protect\ref{def:rot_Rs}}}
\newglossaryentry{Ht}{%
	type=letter,
	name={$H^t(\bbR^d)$},
	description={Sobolev space of order $t\in\bbR^+$},
	origin={Def. \protect\ref{def:Sobolev}}}
\newglossaryentry{Ht_ex_hyp}{%
	type=letter,
	name={$H^t(\bbR^d\!\setminus\!\?h)\!\!\!$},
	description={Functions in \gls{Ht} apart from hyperplane \gls{hyperplane}. Can be extended to finitely many $\{h_i\}_{i=1}^N$.},
	origin={Def. \protect\ref{def:Ht_except_hyp}}}
\newglossaryentry{Hs}{%
	type=letter,
	name={$\Hs(\bbR^d)$},
	description={Sobolev space of functions $f$ such that $\vec s\cdot\nabla f\in L^2(\bbR^d)$},
	origin={Def. \protect\ref{def:Hs}}}
\newglossaryentry{fourier}{%
	type=letter,
	name={$\CF$},
	description={The Fourier transform},
	origin={Eq. \protect\eqref{def:fourier}}}
\newglossaryentry{ball}{%
	type=letter,
	name={$B_\CY(y,r)$},
	plural={$B_{\bbR^d}(0,2^m)$},% trick for def of \gls{Pjlm}
	description={Open ball of radius $r$ in metric space $\CY$, $\set{y'\in \CY}{\dist_\CY(y,y')<r}$}}
\newglossaryentry{heaviside}{%
	type=letter,
	name={$H(\cdot)$},
	plural={$H$},
	description={Heaviside step function, i.e.~$H(y)=\ind_{[0,\infty)}(y)$}}
\newglossaryentry{heaviside_pm}{%
	type=letter,
	name={$H_\pm(\cdot)$},
	description={A step function across a hyperplane \gls{hyperplane}, $H_+(\vec y)=\,$\glspl{heaviside}$(\vec y\cdot \vec n-v)$ in direction of $\vec n$, and vice versa with $H_-(\vec y)=H_+(-\vec y)$},
	origin={Sec. \protect\ref{sec:sing_kappa}}}
\newglossaryentry{advec_discr}{%
	type=letter,
	name={$\VF$},
	sort={F},
	description={Discretisation of the normal equation for \gls{advec_op}},
	origin={Eqs. \protect\eqref{eq:opeqabstractdistcrete}$\&$\protect\eqref{eq:sys_matr_cond}}}
\newglossaryentry{proj_ridge}{%
	type=letter,
	name={$\VP$},
	sort={P},
	description={Compressible projection onto kernel of \gls{advec_discr}},
	origin={Eqs. \protect\eqref{eq:proj_abstract}$\&$\protect\eqref{eq:PMatRep}}}
\newglossaryentry{transl_op}{%
	type=letter,
	name={$T_{\vec y}$},
	description={Translation operator, i.e.~$[T_{\vec y}f](\vec x)=f(\vec x-\vec y)$},
	origin={Eq. \protect\eqref{eq:transl_op_modul_op}}}
\newglossaryentry{modul_op}{%
	type=letter,
	name={$M_{\vec y}$},
	description={Modulation operator (corresponding to definition of \gls{fourier}), i.e.~$[M_{\vec y}f](\vec x) := f(\vec x)\exp(2\pi\ii \vec x\cdot \vec y)$},
	origin={Eq. \protect\eqref{eq:transl_op_modul_op}}}
\newglossaryentry{precond}{%
	type=letter,
	name={$\VW$},
	sort={W},
	description={Diagonal preconditioner in the ridgelet Gel'fand frame (see \gls{gelf_fr_isom}), $\VW=\diag($\gls{weight}$)$},
	origin={Eq. \protect\eqref{eq:precond_matr}}}
\newglossaryentry{weight}{%
	type=letter,
	name={$w_\lambda$},
	sort={Wz},
	description={Weight corresponding to the effect of $\vec s \cdot \nabla$ on \glspl{phi_jlk}, i.e. $w_\lambda:=1+2^j \abs*{\vec s \cdot \sjl}$},
	origin={Eq. \protect\eqref{eq:precond_matr}}}
\newglossaryentry{Delta}{%
	type=letter,
	name={$\Delta$},
	sort={Dz},
	description={In \protect\autoref{sec:int_est}, $\Delta=((c+ad)^2+a^2 b^2)((c-ad)^2+a^2 b^2)$ appears prominently in the partial fraction decomposition of the main integrand (see e.g.~\protect\eqref{app:eq:pfd}). In the rest of the thesis, it denotes the usual Laplacian.},
	origin={Eq. \protect\eqref{app:eq:pfd_Delta}}}
\newglossaryentry{Phi}{%
	type=letter,
	name={$\Phi$},
	description={Usually denotes a frame, i.e.~a collection of functions $\Phi=(\varphi_\lambda)_{\lambda\in\Lambda}$, such that \protect\eqref{eq:framedef} holds. See also analysis and synthesis operators \glspl{analysis_op} and \glspl{synthesis_op}, as well as frame operator \gls{frame_op} and dual frame \gls{Phi_dual}.},
	origin={Subsec. \protect\ref{ssec:prelim_frames}}}
\newglossaryentry{analysis_op}{%
	type=letter,
	name={$G,\,G_\Phi$},
	plural={$G$},% trick to be able to be able to call just one for def of \gls{frame_op}
	sort={Gphi},
	description={Frame analysis operator corresponding to \gls{Phi}},
	origin={Eqs. \protect\eqref{eq:analysis_op}$\&$\protect\eqref{eq:gelfand_frame_dual_op}}}
\newglossaryentry{synthesis_op}{%
	type=letter,
	name={$G^*,\,G_\Phi^*$},
	plural={$G^*$},% trick to be able to be able to call just one for def of \gls{frame_op}
	sort={Gphistar},
	description={Frame synthesis operator corresponding to \gls{Phi}},
	origin={Eqs. \protect\eqref{eq:synthesis_op}$\&$\protect\eqref{eq:gelfand_frame_main_op}}}
\newglossaryentry{frame_op}{%
	type=letter,
	name={$S_\Phi$},
	plural={$S_\Phi^{\protect\phantom{1}}$},% trick to be able to be able to call inverse for def of \gls{Phi_dual}
	sort={Sframe},
	description={Frame operator $S_\Phi=\,$\glspl{synthesis_op}$\,\circ\,$\glspl{analysis_op} corresponding to \gls{Phi}},
	origin={Eq. \protect\eqref{eq:prelim_frame_op}}}
\newglossaryentry{Phi_dual}{%
	type=letter,
	name={$\wt\Phi$},
	description={Canonical dual frame, $\wt\Phi=$\rlap{\glspl{frame_op}}$\protect\phantom{S}_{\protect\phantom{\Phi}}^{-1}$\gls{Phi}},
	origin={Rem. \protect\ref{rem:prelim_dual_frame}}}
\newglossaryentry{lorentz}{%
	type=letter,
	name={$\ell^p_q$},
	description={Lorentz sequence spaces},
	origin={Def. \protect\ref{def:Lorentz}}}
\newglossaryentry{weak_lp}{%
	type=letter,
	name={$\ell^p_w$},
	sort={lorentz_weak},
	description={Special case of \gls{lorentz} with $q=\infty$},
	origin={Def. \protect\ref{def:Lorentz}}}
\newglossaryentry{hyperplane}{%
	type=letter,
	name={$h$},
	%plural={$h_i$},% trick to use for def of \gls{Ht_ex_hyp}
	description={A hyperplane, defined as $\set*{\vec y\in\bbR^d}{\vec y\cdot \vec n=v}$ with normal $\vec n$ and offset $v$},
	origin={Def. \protect\ref{def:Ht_except_hyp}}}
\newglossaryentry{sol_op}{%
	type=letter,
	name={$\CS$},
	sort={S},
	description={The solution operator for the main differential equation, i.e.~the inverse of \gls{advec_op}},
	origin={Sec \protect\ref{sec:sol_op}}}
\newglossaryentry{gelf_fr_isom}{%
	type=letter,
	name={$D_\CH$},
	sort={DH},
	description={Isometry between $\ell^2$ and the sequence space $\CH_\dd$ in the definition of a Gel'fand frame},
	origin={Rem. \protect\ref{rem:gelfand}, \protect\ref{itm:rem:gelfand:additional}}}
\newglossaryentry{Pjl}{%
	type=letter,
	name={$P_\jl$},
	sort={Ph},% should be before Phi/phi/psi
	description={Support of the partition-of-unity function \gls{psi_jl_hat} in frequency space},
	origin={Rem. \protect\ref{rem:Pjl}}}
\newglossaryentry{alpha_j}{%
	type=letter,
	name={$\alpha_j$},
	description={Opening angle of \gls{Pjl} around direction \gls{sjl}; $\alpha_j=2^{-j+1}$},
	origin={Rem. \protect\ref{rem:Pjl}}}
\newglossaryentry{psi_jl_hat}{%
	type=letter,
	name={$\hat \psi_\jl$},
	description={Smooth partition-of-unity function constructed from \gls{Vjl} and \gls{Wrad}, normalised by \gls{Psi}},
	origin={Def. \protect\ref{def:psi_jl}}}
\newglossaryentry{phi_jlk}{%
	type=letter,
	name={$\varphi_\jlk$},
	plural={$\varphi_\lambda$},
	description={Inverse Fourier transform of \gls{psi_jl_hat}, translated by \gls{Ujl}\gls{param_transl}},
	origin={Def. \protect\ref{def:phi_jlk}}}
\newglossaryentry{Vjl}{%
	type=letter,
	name={$V^{(\jl)}$},
	description={Angular window function used to construct \gls{psi_jl_hat}, supported around \gls{sjl} in angle},
	origin={Def. \protect\ref{def:psi_jl}}}
\newglossaryentry{Wrad}{%
	type=letter,
	name={$W$},
	description={Radial window function used to construct \gls{psi_jl_hat}},
	origin={Def. \protect\ref{def:psi_jl}}}
\newglossaryentry{param_lambda}{%
	type=letter,
	name={$\lambda$},
	sort={lz},
	description={Collection of ridgelet parameters $\lambda=($\gls{param_scale},\gls{param_rot},\gls{param_transl}$)$},
	origin={Def. \protect\ref{def:phi_jlk}}}
\newglossaryentry{param_set}{%
	type=letter,
	name={$\Lambda$},
	sort={ly},
	description={Set of indices \gls{param_lambda} --- generic before Def. \protect\ref{def:phi_jlk} and referring to the ridgelet parameters from there on}}
\newglossaryentry{param_scale}{%
	type=letter,
	name={$j$},
	sort={j},
	description={Scale of a ridgelet, corresponding to frequency support of underlying \gls{psi_jl_hat} near radius $\sim 2^j$},
	origin={Def. \protect\ref{def:psi_jl}}}
\newglossaryentry{param_rot}{%
	type=letter,
	name={$\ell$},
	sort={l},
	description={Parameter numbering the different directions \gls{sjl} on a given scale \gls{param_scale}},
	origin={Def. \protect\ref{def:psi_jl}}}
\newglossaryentry{param_transl}{%
	type=letter,
	name={$\vec k$},
	sort={k},
	description={Translation in physical space used in definition of \gls{phi_jlk}, after transformation by \gls{Ujl}},
	origin={Def. \protect\ref{def:phi_jlk}}}
\newglossaryentry{sjl}{%
	type=letter,
	name={$\sjl$},
	description={In terms of the angle, each $\sjl$ is the center of one \gls{Pjl}. On scale \gls{param_scale}, $\cup_\ell \sjl$ is an approximately uniform sampling of $\bbSd$, with average distance $2^{-j}$ between neighbours $\sjl$ and $\sjld$.},
	origin={Def. \protect\ref{def:psi_jl}}}
\newglossaryentry{Ujl}{%
	type=letter,
	name={$U_\jl$},
	plural={$U_\jl^{\protect\phantom{1}}$},
	description={Transformation acting on \gls{param_transl} in the definition of \gls{phi_jlk}, $U_\jl=\,$\rlap{\glspl{Rjl}}$\protect\phantom{R}_{\protect\phantom{\jl}}^{-1}$\glspl{Da}},
	origin={Def. \protect\ref{def:phi_jlk}}}
\newglossaryentry{bbRp}{%
	type=letter,
	name={$\bbR^+$},
	sort={R},
	description={Strictly positive real numbers, $(0,\infty)$}}
\newglossaryentry{bbRpz}{%
	type=letter,
	name={$\bbR^+_0$},
	sort={Ra},
	description={Positive real numbers, $[0,\infty)$}}
\newglossaryentry{bbN}{%
	type=letter,
	name={$\bbN$},
	sort={N},
	description={Natural numbers, not including zero}}
\newglossaryentry{bbNz}{%
	type=letter,
	name={$\bbN_0$},
	sort={Na},
	description={Natural numbers, including zero}}
\newglossaryentry{Rjl}{%
	type=letter,
	name={$R_\jl$},
	plural={$R_\jl^{\protect\phantom{1}}$},% trick to be able to be able to call inverse for def of \gls{Ujl}
	description={Transformation \gls{Rs} corresponding to $\vec s=\,$\gls{sjl}},
	origin={Def. \protect\ref{def:phi_jlk}}}
\newglossaryentry{Da}{%
	type=letter,
	name={$D_a$},
	plural={$D_{2^j}$},
	description={Matrix dilating the first component of a vector by factor $a$},
	origin={Def. \protect\ref{def:phi_jlk}}}
\newglossaryentry{alpha_j_m}{%
	type=letter,
	name={$\alpha_j^m$},
	description={Opening angle of \gls{Pjlm} around \gls{sjl}},
	origin={Eq. \protect\eqref{eq:est_alpha_j_m}}}
\newglossaryentry{Pjlm}{%
	type=letter,
	name={$P_\jl^m$},
	sort={Pha},
	description={Minkowski sum of \gls{Pjl} and \glspl{ball}},
	origin={Def. \protect\ref{def:Pjlm}}}
\newglossaryentry{Qjlm}{%
	type=letter,
	name={$Q_\jl^m$},
	description={Set difference between $P_\jl^{m+1}$ and \gls{Pjlm}},
	origin={Def. \protect\ref{def:Pjlm}}}
\newglossaryentry{Imn}{%
	type=letter,
	name={$I_{m,n}$},
	description={Main object of study in App. \protect\ref{sec:int_est}},
	origin={Thm. \protect\ref{th:Imn_est}}}
\newglossaryentry{base_canonical}{%
	type=letter,
	name={$\vec e_i$},
	sort={ei},
	plural={$\vec e_1$},
	description={Canonical basis of $\bbR^d$ with $\vec e_1$ having a one in its $i$\nth component and zeros elsewhere}}
\newglossaryentry{Psi}{%
	type=letter,
	name={$\Psi$},
	description={Sum of all (squared) window functions in frequency, used to normalise in definition of \gls{psi_jl_hat}},
	origin={Def. \protect\ref{def:psi_jl}}}
\newglossaryentry{psi_jl_ref}{%
	type=letter,
	name={$\hat\psi_{(\jl)}$},
	description={Transformation of \gls{psi_jl_hat} by \rlap{\glspl{Ujl}}$\protect\phantom{U}_{\protect\phantom{\jl}}^{-\top}$ to reference area},
	origin={Eq. \protect\eqref{eq:psi_trafo}}}
\newglossaryentry{kappa}{%
	type=letter,
	name={$\kappa$},
	description={Absorption coefficient in \gls{advec_op}},
	origin={Eq. \protect\eqref{eq:LinTrans_intro}}}
\newglossaryentry{proj_hyp}{%
	type=letter,
	name={$\CP_{\vec y}$},
	sort={Phb},
	description={Projection onto hyperplane orthogonal to $\vec y$ (normalised), i.e.~$\CP_{\vec y} \vec x=\vec x-(\vec x \cdot \vec y) \vec y$},
	origin={Lem. \protect\ref{lem:fourier_decomp}}}
\newglossaryentry{alpha_lambda}{%
	type=letter,
	name={$\alpha_\lambda$},
	description={An element of the sequence $\inpr{\varphi_\lambda,f}$ for an $f\in\,$\gls{Ht_ex_hyp}},
	origin={Prop. \protect\ref{prop:loc_angle}}}
\newglossaryentry{alpha_lambda_rs}{%
	type=letter,
	name={$\alpha_\lambda^{\rmr},\,\alpha_\lambda^\rms$},
	description={A split of \gls{alpha_lambda} into regular and singular component according to \protect\eqref{eq:fourier_decomp}},
	origin={Prop. \protect\ref{prop:loc_angle}}}
\newglossaryentry{beta_lambda}{%
	type=letter,
	name={$\beta_\lambda$},
	description={An element of the sequence $\langle\varphi_\lambda,\,$\gls{sol_op}$[f]\rangle$ for an $f\in\,$\gls{Ht_ex_hyp}},
	origin={Prop. \protect\ref{prop:loc_angle}}}
\newglossaryentry{beta_lambda_rs}{%
	type=letter,
	name={$\beta_\lambda^{\rmr},\,\beta_\lambda^\rms$},
	description={A split of \gls{beta_lambda} into regular and singular component according to \protect\eqref{eq:fourier_decomp}},
	origin={Prop. \protect\ref{prop:loc_angle}}}
\newglossaryentry{transl_sh}{%
	type=letter,
	name={$\vec t(\vec k)$},
	description={Shifted translation $\vec t(\vec k)=\,$\gls{param_transl}$\,-v$\rlap{\glspl{Ujl}}$\protect\phantom{U}_{\protect\phantom{\jl}}^{-1}\vec n$, with $\vec n$ and $v$ corresponding to \gls{hyperplane}},
	origin={Prop. \protect\ref{prop:loc_space}}}
\newglossaryentry{rho_one_two}{%
	type=letter,
	name={$\rho_1,\,\rho_2$},
	sort={Rz},
	description={Intermediate quantities based on \gls{transl_sh}},
	origin={Prop. \protect\ref{prop:loc_space}}}
\newglossaryentry{theta_jl}{%
	type=letter,
	name={$\theta_\jl(\vec n)$},
	sort={Tz},
	description={Angle between $\sjl$ and $\vec n$, $\theta_\jl(\vec n)=\arccos(\sjl\cdot\vec n)$},
	origin={Prop. \protect\ref{prop:loc_angle}}}
\newglossaryentry{param_set_angle}{%
	type=letter,
	name={$\Lambda^j_r(\vec n)$},
	sort={lyy},
	description={Subset of $\lambda\in \Lambda$ such that $\sin\,$\gls{theta_jl} is in a given interval},
	origin={Eq. \protect\eqref{eq:Lambda_jr}}}
\newglossaryentry{Tjl}{%
	type=letter,
	name={$T_\jl$},
	description={The tail of translations \gls{param_transl} away from \gls{transl_sh} under a suitable transformation},
	origin={Eq. \protect\eqref{eq:approx_main_sing_tail}}}
\newglossaryentry{idmatr}{%
	type=letter,
	name={$\bbI_k$},
	description={Identity matrix of size $k\times k$}}
\newglossaryentry{SigmaPhi}{%
	type=letter,
	name={$\Sigma_N(\Phi)$},
	sort={Sy},
	description={The non-linear space of functions comprised of linear combinations of $N$ elements of \gls{Phi}},
	origin={Eq. \protect\eqref{eq:SigmaN_Phi}}}
\newglossaryentry{Ck}{%
	type=letter,
	name={$\CC^k$},
	description={Classical smoothness space of order $k$},
	origin={Def. \protect\ref{def:smoothness_Ck}}}
%\newglossaryentry{}{%
%	type=letter,
%	name={$ $},
%	description={ },
%	origin={ \protect\ref{ }}}
%\newglossaryentry{}{%
%	type=letter,
%	name={$ $},
%	description={ },
%	origin={ \protect\ref{ }}}


\newcommand{\grayy}{{\color{gray!75}y}}
\newcommand{\grayyvec}{{\color{gray!75}\vec y}}
\newcommand{\grayymat}{{\color{gray!75}\VY}}
\newcommand{\grayyset}{{\color{gray!75}\CY}}

\newglossaryentry{a_minmax}{%
	type=symbol,
	name={$\grayy_<,\,\grayy_>$},
	description={Minimum and maximum of two quantities (usually primed and unprimed, respectively); i.e.~$y_<:=\min(y,y')$, $y_>:=\max(y,y')$},
	origin={Sec. \protect\ref{sec:notation}}}
\newglossaryentry{l_regabs}{%
	type=symbol,
	name={$\reg{\grayyvec}$},
	description={Regularised absolute value (to avoid problems with dividing by zero), $\langle\vec y\rangle:=\sqrt{1+|\vec y|^2}$},
	origin={Sec. \protect\ref{sec:notation}}}
\newglossaryentry{s_indicator}{%
	type=symbol,
	name={$\ind_{\grayyset}$},
	description={Indicator function for a given set $\CY$}}
\newglossaryentry{s_complement}{%
	type=symbol,
	name={$\grayyset^\compl$},
	description={Complement of $\CY$ in ambient space},
	origin={}}
\newglossaryentry{f_hat}{%
	type=symbol,
	name={$\hat\grayy$},
	description={Shorthand notation for \gls{fourier}$[y]$ for a function $y$},
	origin={}}
\newglossaryentry{l_prime}{%
	type=symbol,
	name={$\grayyvec'$},
	description={For vectors in Chapters \ref{ch:prop_advec} and \ref{ch:approx}, $i$ primes denote all but the first $i$ entries of a vector, i.e.~$\vec k{}'=(k_2,k_3,\ldots)^\top$},
	origin={}}
\newglossaryentry{l_top}{%
	type=symbol,
	name={$\grayyvec^\top,\,\grayymat^\top$},
	description={Transpose of $\vec y$ resp.~$\VY$},
	origin={}}
\newglossaryentry{l_bracket}{%
	type=symbol,
	name={$[\grayyvec]$},
	description={Linear span of $\vec y$, with obvious extension to $[\vec y_1,\vec y_2,\ldots]$},
	origin={Sec. \protect\ref{sec:notation}}}
\newglossaryentry{s_bot}{%
	type=symbol,
	name={$\grayyset^\bot$},
	description={Orthogonal complement of $\CY$},
	origin={Sec. \protect\ref{sec:notation}}}
\newglossaryentry{a_bar}{%
	type=symbol,
	name={$\overline{\grayy}$},
	description={Complex conjugate of $y$},
	origin={}}
\newglossaryentry{a_ceil}{%
	type=symbol,
	name={$\ceil{\grayy}$},
	description={Rounding $y$ up to the nearest integer},
	origin={}}
\newglossaryentry{a_floor}{%
	type=symbol,
	name={$\floor{\grayy}$},
	description={Rounding $y$ down to the nearest integer},
	origin={}}
\newglossaryentry{m_lld}{%
	type=symbol,
	name={$\grayymat_\lld$},
	description={Matrix coefficient of $\VY$ with row index $\lambda$ and column index $\lambda'$},
	origin={}}
\newglossaryentry{coeff}{%
	type=symbol,
	name={$[\grayy^n] {\color{gray!75}f}$},
	description={Operator extracting the $n$\nth Taylor coefficient in $y$ from $f$ around zero},
	origin={Eq. \protect\eqref{app:eq:def_coeff_op}}}
\newglossaryentry{m_approximand}{%
	type=symbol,
	name={$\grayymat^{[k]}$},
	description={The $k$\nth approximand for $\VY$ from the definition of compressibility},
	origin={Def. \protect\ref{def:compr}}}
\newglossaryentry{s_card}{%
	type=symbol,
	name={$\#\grayyset$},
	description={Cardinality of $\CY$},
	origin={}}
%\newglossaryentry{m_psparse}{%
%	type=symbol,
%	name={$\norm{\grayymat}_{\psp}\!\!\!$},
%	description={Measure of $p$-sparsity of $\VY$},
%	origin={Def. \protect\ref{def:sparse}}}
\newglossaryentry{f_snorm}{%
	type=symbol,
	name={$\snorm{\grayy}_{\CC^k}$},
	description={Point-wise maximum of all derivatives of a function $y$ up to order $k$},
	origin={Def. \protect\ref{def:smoothness_Ck}}}
%\newglossaryentry{}{%
%	type=symbol,
%	name={$ $},
%	description={ },
%	origin={}}
%\newglossaryentry{}{%
%	type=symbol,
%	name={$ $},
%	description={ },
%	origin={}}
